Combining Vagueness Detection with Deep Learning to Identify Fake News

In this paper, we combine two independent detection methods for identifying fake news: the algorithm VAGO uses semantic rules combined with NLP techniques to measure vagueness and subjectivity in texts, while the classifier FAKE-CLF relies on Convolutional Neural Network classification and supervised deep learning to classify texts as biased or legitimate. We compare the results of the two methods on four corpora. We find a positive correlation between the vagueness and subjectivity measures obtained by VAGO, and the classification of text as biased by FAKE-CLF. The comparison yields mutual benefits: VAGO helps explain the results of FAKE-CLF. Conversely FAKE-CLF helps us corroborate and expand VAGO's database. The use of two complementary techniques (rule-based vs data-driven) proves a fruitful approach for the challenging problem of identifying fake news.

==> FUSION_ expert-based Vago and deep-based FakeClf for desinfo/texts/1intro.tex <==
 
 
The computational verification of textual claims is motivated by the  proliferation of misinformation on the Web and online resources. Such methods are needed because human verification does not scale up to the diffusion speed of online misinformation, which spreads up to six times faster than real news~\cite{Vosoughi1146}. It is also worth mentioning that up to 50\% of the shares of viral claims happens within minutes of their appearance~\cite{DBLP:journals/corr/abs-1304-6777}.


 Extant proposals for detecting fake news have been focused on verifying textual claims given reference information, based on corpora of previously checked claims~\cite{TchechmedjievFB19,ShaarBMN20}. Some approaches exploit the thousands of reports written by journalists in fact-checking organizations to automatically verify if a claim is true or not. Other works use textual documents as trusted information to be analyzed in order to validate claims. Recently, there have been new methods to verify claims using reference-structured data, for example by adapting transformers to let them model datasets~\cite{ChenWCZWLZW20,tapas20}. 


In this paper, we propose to
treat lexical vagueness as a cue for the automatic identification of fake news conveying biased information. The motivation is twofold: vague claims are less sensitive to factual refutation than precise claims \cite{Egre&Icard2018}; moreover vague terms are more prone to subjective interpretation than precise terms, particularly in the adjectival domain \cite{Kaiser&Wang2021}.
On the technical side, we use and compare two independent detection methods for identifying fake news: the first, deployed in the algorithm \vago, detects and measures vagueness and subjectivity in texts using a semantic-based approach combined with NLP techniques, while the second, deployed in the classifier \fake, relies on Convolutional Neural Network to classify texts as biased or legitimate. The motivation behind this comparison is to investigate whether \vago's and \fake's respective classification results actually converge. Our aim is thus to confront and to relate a semantic method with a deep-learning method and to pool their results. 


The paper is organized as follows. In section \ref{sec:vago}, we present the expert-based approach of \vago. We first motivate our emphasis on vagueness by explaining the way in which some vague expressions convey subjectivity. We present a typology of vague terms used by \vago to classify corpora as being either \textit{vague} or \textit{precise}, \textit{opinion} or \textit{factual}, as well as simple scoring rules used to implement an online text analyzer. 



Section \ref{sec:deep} describes the deep-learning approach of \fake. This classifier based on a Convolutional Neural Network (CNN) architecture was trained on more than 36,000 texts manually labelled as ``fake news'' or ``legitimate''. \fake exploits Class Activation Maps (CAMs) to define the contribution of each sub-part of the document to each considered class, allowing for word-level interpretation. 

In section \ref{sec:correlation}, we compare the categorization by \vago between \textit{vague} or \textit{precise}, \textit{opinion} or \textit{factual}, with the classification of news articles by \fake between \textit{legitimate} or \textit{biased}. 
In terms of explainable AI, we expect that doing so will help us see more clearly into the determinants of the \fake classification. 


Finally, in Section \ref{sec:discussion} we discuss the opportunities and gains in terms of explainability of mixing expert-based systems with deep-learning, data-driven classifiers. 

==> FUSION_ expert-based Vago and deep-based FakeClf for desinfo/texts/2vago.tex <==

\subsection{Vagueness and subjectivity}



Vague words are expressions whose meaning is indeterminate and compatible with an open-ended range of possible interpretations\cite{russell1923vagueness}. Typical examples of vague words include gradable adjectives like ``tall'', ``rich'', ``intelligent'', whose extension is left open by the speaker \cite{kennedy2007vagueness}. When hearing ``John is tall'', the listener generally cannot infer a precise representation of John's height, but only a set of more or less probable values \cite{lassiter2017adjectival}. This is different if we hear the precise sentence ``John is exactly 187cm tall'', which eliminates more possibilities. 

There is no direct relation between a sentence being vague and its classification as true or false
%There is no direct relation between vagueness and either truth or falsity
%There is no direct relation between a sentence being vague and its being false \emph{simpliciter} as opposed to true \emph{simpliciter}
\cite{Egre&Icard2018}. An utterance with precise truth conditions can perfectly be false (``the Eiffel Tower is 96 meters high''). Conversely, a vague sentence can be judged uncontroversially true (``the Eiffel Tower is a tall building''). As noted by \cite{russell1923vagueness}, however, a vague sentence has higher chances of being judged true than a precise one, because it is compatible with more possible states of affair. Relatedly, vague expressions are generally seen as more subjective than precise expressions, because both speaker and listener can interpret them in different ways \cite{verheyen2018subjectivity}. Thus, a large class of gradable adjectives is described as subjective, or even as evaluative \cite{kennedy2013two,mcnally2017aesthetic,Solt2018,Kaiser&Wang2021}.


In principle, a seasoned liar could use only precise language to create fake news. But it may be harder to ensure coherence, and it may thereby add up to the cognitive cost of having to make up a story  (see \cite{verschuere2018taxing}). In contrast, using vague language can be a cheap way of making one's utterances easier to accept, because less sensitive to factual refutation \cite{Egre&Icard2018}. Importantly, vague language is also used cooperatively to minimize error and to communicate uncertainty \cite{deemter2009utility,Egre&Icard2018, egre2020optimality}. But an overwhelming reliance on vague language may signal that the discourse is possibly less factual, and more prone to \emph{bullshitting} (see \cite{Frankfurt2009}) or to the spreading of \textit{biased} information.



\subsection{A typology of vague expressions}

To detect vagueness and subjectivity in texts, IJN and Mondeca have developed a lexical database and associated algorithm called \texttt{VAGO}.
The inventory relies
on the typology proposed in \cite{Egre&Icard2018}, which distinguishes four types of lexical vagueness: approximation ($V_A$), generality ($V_G$), degree-vagueness ($V_D$), and combinatorial vagueness ($V_C$). 

Expressions of approximation here include mostly modifiers such as ``around'', ``about'', ``almost'', ``nearly'', ``roughly'', which loosen up the meaning of the expression they modify (compare ``around 10 o'clock" and ``10 o'clock"). Expressions of generality include determiners such as ``some'' and modifiers like ``at most'', ``at least''. Unlike the former, these expressions have precise truth-conditions but they fail to give a maximally informative answer to the question ``how many'' (compare ``some students/at least three students left'' to ``eleven students left''). 

The class of degree-vague and combinatorially vague expressions includes mostly one-dimensional adjectives on the one hand (like ``tall'', ``old'', ``large'') and multi-dimensional adjectives on the other (``beautiful'', ``intelligent'', ``good'', ``qualified''), which combine several dimensions or respects of comparison. The opposition between degree-vagueness and combinatorial vagueness is adapted from \cite{alston1964philosophy}. %: degree-vague adjectives are linked to physical magnitudes for which there is a standard measurement scale (e.g. cm for height, years for age), unlike combinatorially vague adjectives. 
In Alston's approach, combinatorial vagueness concerns not just adjectives but also common nouns and verbs. The class of degree-vague and combinatorially vague expressions consists mostly of adjectives in \vago (see Section \ref{sec:correlation}), knowing that in the case of adjectives, the \emph{degree} vs \emph{combinatorial} distinction is congruent with the distinction proposed by Kaiser and Wang between \emph{simple-subjective} vs \emph{complex-subjective} adjectives \cite{Kaiser&Wang2021}.

Thus, we assume that subjectivity is introduced foremost by expressions of type $V_D$ and $V_C$. Two competent speakers can have a non-factual disagreement as to whether someone is ``tall'' or ``old'', regardless of the existence of common scales of physical measurement, and even as they share the same knowledge of height or age \cite{kennedy2013two}. And the more dimensions attached to an expression, the more disagreement is expected to arise between competent speakers, as evidenced in the case of evaluative adjectives like ``beautiful'' or ``smart'' for which no standard scale of measurement is available \cite{mcnally2017aesthetic}. By contrast, we assume that expressions of type $V_A$ and $V_G$ give rise to no subjectivity, or at least to limited subjectivity, since the interpretation of these expressions is number-relative and less context-sensitive (``roughly 20'' is relative to the precise value 20, unlike ``tall'', and similarly ``some students'' literally means ``more than 0 students'').

As a result, expressions of type $V_A$ and $V_G$ are treated as factual expressions, and expressions of type $V_D$ and $V_C$ as subjective expressions. This means that logically the class of vague expressions is not coextensional with the class of subjective expressions, but forms a superset.

%This means that we do not handle the class of vague expressions as coextensional with the class of subjective expressions. 

%In our database, we ended up including many more terms of type $V_D$ and $V_C$ compared to $V_A$ and $V_G$. Practically, however, we can calculate two separate scores for sentences: a score of vagueness vs. precision, and a score of subjectivity vs objectivity (opinion vs factual).


\subsection{VAGO: detection and scoring}



%Based on the connection between vagueness and subjectivity, IJN and Mondeca have developed a lexical database and associated algorithm called \texttt{VAGO}, intended to provide a measure of the relative vagueness of discourse.

In \vago, vagueness and subjectivity are detected and scored bottom-up, from words to sentences to larger texts. 
%\texttt{VAGO} rests on a syntactic parser and provides semantic markers.
For a given sentence, its vagueness score  is defined simply as the ratio of vague words to the total number of words of the sentence.


\begin{equation}
R_{vague}(\phi) =
\frac{(\overbrace{|V_G|_{\phi} + |V_A|_{\phi}}^{factual} + \overbrace{|V_D|_{\phi} + |V_C|_{\phi}}^{subjective})}{N_{\phi}}
\end{equation}

\noindent where $N_{\phi}$ designates the total number of words in the sentence $\phi$ and $|V_G|_{\phi}$, $|V_A|_{\phi}$, $|V_D|_{\phi}$ and $|V_C|_{\phi}$ denote the number of terms of each of the four types of vagueness (generality, approximation, degree-vagueness and combinatorial vagueness).

 
Similarly, the subjectivity score of a sentence is calculated as the ratio of subjective expressions to the total number of words in the sentence.

\begin{equation}
R_{subjective}(\phi) =
\frac{|V_D|_{\phi} + |V_C|_{\phi}}{N_{\phi}}
\end{equation}

\noindent Both the vagueness score and the subjectivity score of a sentence vary between 0 and 1. When a sentence contains at least one vague term, the degree of {vagueness} of the sentence is nonzero, $R_{vague}(\phi) > 0$. When $R_{vague}(\phi)=0$ this implies the sentence does not contain vague vocabulary, and similarly for subjectivity. 



For sets of sentences, the vagueness score and the subjectivity score can be defined as the proportion of sentences with nonzero vagueness and nonzero subjectivity scores respectively. More fine-grained measures can be proposed, but these scores suffice to characterize the prevalence of each feature. If $T$ is a text and $N_T$ its total number of sentences, then:

\begin{equation}\label{eq:prop_vague}
R_{vague}(T)=\frac{|\{\phi \in T | R_{vague}(\phi)>0\}|}{N_T}
\end{equation}

\begin{equation}\label{eq:prop_subj}
R_{subjective}(T)=\frac{|\{\phi \in T | R_{subjective}(\phi)>0\}|}{N_T}
\end{equation}

\subsection{VAGO Implementation}
\texttt{VAGO}'s back-end is built on top of the popular GATE~\cite{gatearch} framework for NLP content processing. It also leverages the semantic content annotator CA-Manager~\cite{cam2013}, a semantic-based tool for knowledge extraction from unstructured data. The current pipeline automatically detects the language of the corpus (English or French) using TexCat.\footnote{\url{https://www.let.rug.nl/vannoord/TextCat/index.html}} 

The back-end uses a workflow composed of different analysis engines, combining NLP processing from GATE and semantic technologies with a UIMA-based infrastructure.\footnote{Unstructured Information Management Architecture (\url{http://uima.apache.org)}} UIMA architecture allows enriching and customizing engines to address specific needs in the application. \texttt{VAGO} is also available through HTTP REST API. 

\subsection{Online tool}

The online tool \texttt{VAGO}, available from Mondeca's website,\footnote{\url{https://research.mondeca.com/demo/vago/}} provides a graphical interface for the representation of these scores using two barometers. One barometer represents the degree to which a text is vague or precise. The other barometer indicates the degree to which the text reports an opinion or is factual (the proportion of subjective vs objective vocabulary). A section of detailed results explains for each sentence the vague triggers detected and the corresponding category ($V_X$). 

The online tool uses an anonymous profile, with some restrictions to call the service such as a limit number of characters as input (e.g., 1200), and some predefined short sample texts. The online application automatically detects the language of the text entered by the user (French or English). 



As a toy example, consider the text $T=\{$``\emph{Most sensational news articles are sometimes hard to believe'', ``Two plus two equals four'', ``Mary left Paris around 2pm''}$\}$, comprised of three sentences. $T$ contains five vague terms (``most'', ``sensational'', ``sometimes'', ``hard", ``around''), with ``sometimes'' and ``most'' instantiating generality, ``sensational'' and ``hard" pertaining to combinatorial vagueness, and ``around'' to approximation. While the sentence ``\emph{Two plus two equals four''} is precise, the other two are vague: \emph{``Mary left Paris around 2pm''} is only factual but ``\emph{Most sensational news articles are sometimes hard to believe''} contains both factual and subjective terms. The barometers reporting the proportion of vague and subjective sentences in the text $T$ are shown in Figure \ref{fig:barometers}.   

\begin{figure}[H]
\captionsetup[subfigure]{labelformat=empty}
   \includegraphics[width=0.49\textwidth]{figures/Barometers}
    \caption{Results summary for text with three sentences}
    \label{fig:barometers}
\end{figure} 



==> FUSION_ expert-based Vago and deep-based FakeClf for desinfo/texts/3deep.tex <==
 
    
Another way to detect fake news is to learn how to distinguish them inductively, by means of examples. In this section we detail a previously developed classifier \cite{gadek2020interpretable}, \fake, and the datasets used for training.
    
\subsection{Deep learning text classification: Related work }
    
    Part of machine learning, text classification is known through numerous applications: sentiment analysis \cite{abbasi_sentiment_2008}, language identification \cite{castro_smoothed_2017} or even emotion detection \cite{liu2019oasis}, dealing with a variety of texts from tweets to Wikipedia articles.
    While very efficient, these methods often lack explainability as most of them work in a ``black box'' mode.
    
Explaining a prediction on a text means to characterize sub-document segments: this can be performed either by observing the behavior of an attention mechanism \cite{bahdanau_neural_2014}; another way relies on the extraction of class activation maps \cite{zhou_learning_2016}. 

%To let the model manage itself its attention,

Regarding the first approaches, a self-attention mechanism was introduced in \cite{lin_structured_2017} for text classification. %where attention scores assigned to crucial words are measured. %Also, it has been shown that attention is transferable \cite{zagoruyko_paying_2017}. 
Attention scores are computed as the salience of a sub-part of the document relatively to a generic classification task, and not relatively to a precise label. Indeed this mechanism focuses on the ``important'' words, not on the words that justify an isolated prediction. Ranging from 0 (no interest) to 1 (high interest), the attention scores do not carry information about the prediction. However, high-attention words and phrases act with more impact, either for or against class membership.

The second approach, \textit{class activation maps} (CAMs), was introduced in \cite{zhou_learning_2016}. CAMs are literally the contribution of each sub-part of the document to each considered class. %They are extracted by exploiting the features produced by the penultimate neuron layer.
In order to preserve a direct link with the input, CAMs require specific architecture conditions detailed in the next paragraph. 

\subsection{CAM to explain text classification}
\label{sec:cam}
CAMs were first introduced in image classification \cite{zhou_learning_2016}, and only recently adapted to text classification \cite{guelorget_deep_2020}. The intuition relies on the fact that spatiality is preserved across convolutional layers, whereas it is lost in the last fully-connected layers used in most classifiers. Thus this method concerns fully-convolutional networks; the final prediction layer can rely either on global average pooling (GAP) or on global max pooling (GMP), which is applied to squash the $T$ spatial features vectors associated to the deepest feature maps $F = \{ F_1, ..., F_T \} \in \mathbb{R}^{T \times K}$ into a single, global feature vector $F_g\in\mathbb{R}^K$ in which all spatiality is lost. $K$ denotes the size of the considered feature maps. 

The technical details of the \fake model implementation are the following: it consists of a fully-convolutional neural network made of 3 layers of 128 kernels of size 5. The final layer consists of a global average pooling and a softmax classification. As inputs, we rely on a pre-trained word embedding, of dimension 300: FastText \cite{joulin_bag_2016}. Indeed, a more recent embedding, even if context-aware such as BERT \cite{devlin_bert:_2018} or Elmo \cite{peters_deep_2018}, would mean a much higher-complexity architecture, detrimental to the interpretability of the class prediction (as it would take into account the role of the neighboring words without explaining how). The texts are only tokenized (words and punctuation items) through the Python library NLTK\footnote{\url{https://www.nltk.org/}}. These pre-trained embeddings imply that the model has to grasp the context: \fake does it thanks to its convolutional layers. Note that \fake traces the importance of each token's contribution.

Because CAMs require to preserve the temporality across layers, \fake uses the same padding for all convolutions to have exactly one output layer directly corresponding to each input token. As a result the last convolutional layer presents a number of outputs that is equal to the number of input words: the $t^{th}$ output of the last convolutional layer describes the $t^{th}$ word of the input sentence, considering also its context within the convolutional receptive field. 

The CAM extraction is explained hereafter. If there are $C$ different labels, then the softmax input is defined as:

\begin{equation}
S = W^TF_g + b
\end{equation}

\noindent where $W = \{w_c^k\} \in \mathbb{R}^{K\times C}$ and $b\in \mathbb{R}^C$ are the final weights and biases.
For any input example $x$, the class activation map for label $c$ at location $t$ is obtained by summing the contribution $w_c^kF_t^k$ of each scalar feature $F_t^k$ to the final score of label $c$, as described in the following equation:

\begin{equation}
\label{eq:CAM-definition}
\text{CAM}(x,c,t) = \sum_k{w_c^k F_t^k}
\end{equation}

% CAMs address the aforementioned limitations of the attention scores to fulfill our purpose:
As a result, in a text classification context, CAMs provide a signed contribution score of each word (or punctuation item) to each class membership tackled by the model. 
% Hence, we chose to use CAMs to extract dense, comprehensive knowledge from a network previously trained on a large set of documents. 
%, thus $R = \text{CAM}$. 
Our CAM-extracted model is illustrated in Figure~\ref{fig:schema2}.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/network.pdf}
	\caption{Extraction of Class Activation Maps from a tokenized sentence, from \cite{gadek2020interpretable}.}
	\label{fig:schema2}
\end{figure}

%The input of our model is a list of tokens, which are converted to their embeddings. Three convolutional layers enable the model to fully grasp the sentence structure, each one with a kernel size of 5. Afterwards, for each class, each tensor $F_i$  ...
%\textit{comment the figure: inputs, throughput, output & CAMs. Assert that the global average pooling strategy gives less importance to a given word, thus lowering the weight of a keyword and furthering the classifier from a bag-of-words.}

\subsection{Predicting fake-like news articles}
We trained this CAMs-based architecture to detect ``fake news'', using the following well-known press articles datasets:

\begin{itemize}
    \item Kaggle fake news\footnote{\url{https://www.kaggle.com/mrisdal/fake-news}} is composed of 13,000 documents in English, tagged as ``fake'': either ``\textit{biased}'' or ``\textit{bullshit}''. We decided to merge these two ``fake'' categories under a single ``\textit{biased}'' label as the first iterations of this classifier did not distinguish well these two kinds of bad-quality content. Moreover, doing so enables the aggregation with the next datasets.
    
    \item ISOT\footnote{\url{https://www.uvic.ca/engineering/ece/isot/datasets/fake-news/index.php}} contains 21,417 ``true'' and 23,481 ``fake'' articles, subsequently referred to as ISOT-True and ISOT-Fake.
    
    \item SignalMedia1M\footnote{\url{http://research.signalmedia.co/newsir16/signal-dataset.html}} gathers a huge corpus of press articles (in English), deemed to be legitimate \cite{katsaros2019machine}. From this resource, we select two random samples:
    \begin{itemize}
        \item 15,064 articles to balance the training,% of the classifier,
        \item 20,071 other articles for the evaluation part.
    \end{itemize}
    
    %\textcolor{blue}{PE: do we mean the three classes?Rewrite to explain that we want fake vs legitimate be balanced across the 3 corpora}
\end{itemize}
On Kaggle and ISOT, a random train/test split policy is applied (80\%/20\%). The resulting datasets are then aggregated with their SignalMedia1M complement. 

% The use of contextualized embeddings such as BERT \cite{devlin_bert:_2018} or Elmo \cite{peters_deep_2018} would be a return to the ``black box'' phenomenon, because they exploit the whole text to embed each token and lack any explanability features. Our inputs rely on the \textit{fasttext} pre-trained embeddings, of dimension 300. The texts are only tokenized (including the punctuation) through the Python library NLTK\footnote{\url{https://www.nltk.org/}}. These pre-trained embeddings imply that the model has to grasp the context: \fake does it thanks to its convolutional layers.


A recurrent objection on fake news classification is the risk to overfit the classifier on a topic-specific dataset, over-focusing on a few words. Particularly hard to analyze, this problem stems from the scarcity of similarly-labeled, thematically different datasets. \fake presents an advantage in order to investigate this point, through the class activation mappings: high-score tokens are easily identified.

\subsection{Validating the classifier on unseen data}

The training dataset of \fake consists of the four corpora previously listed (ISOT-True, ISOT-Fake, SignalMedia1M, Kaggle). The measure of the model performance with respect to the four corpora is presented on Figure \ref{fig:clf_results_per_source}. The y-axis is the output score; 0 means \textit{legitimate} while 1 stands for a \textit{biased} content. The x-axis shows the source corpora. The letter-value plots\footnote{The widest box stretches between the first and last quartiles, the second widest boxes stretch between the first/last quartile and the first/last octile, the third widest between the first/last octile and the first/last hexadeciles, and so forth \cite{letter-value-plot}.} illustrate the distribution of articles that were part of the test dataset (20\% of total data, excluded from the training set).

ISOT-True and ISOT-Fake are two facets of the ISOT dataset. ``True'' news, labeled as \textit{legitimate} articles, and ``fake'' articles, labeled as \textit{biased}, are very well recognized and separated. The same trend is also remarkable in separating SignalMedia1M and Kaggle's datasets, even though the latter shows a fuzzier distribution. Overall the classification performance on these {test} datasets results in an F1-score $= 0.955$, indicative of high accuracy. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/clf_results_per_source.pdf}
    \caption{Classification of source corpora in the \textit{test} dataset as \textit{legitimate} (0) or \textit{biased} (1) by \fake.%\textcolor{blue}{Figure could be improved: legitimate texts could be grouped left, and biased right? or same color code as below could also be used instead of separate color for each corpus?} %(letter-value plots)
    }
    \label{fig:clf_results_per_source}
\end{figure}



==> FUSION_ expert-based Vago and deep-based FakeClf for desinfo/texts/4comparison.tex <==

%figures "boxplot", description factuelle, éléments d'interprétation.
%idéalement, un exemple de résultat (de Vago ; de Fake) est déjà présent dans les parties précédentes.
% il faut une section qui presente le corpus utilisé, la version des dicos de VAGO 

We now turn to the comparison between the classification obtained by \fake and the measures produced by \vago.

\subsection{Experimental Settings}
% todo: Add the description of the full database of VAGO 

The lexicon used by \vago at the time of this experiment consisted of $1,527$ English terms, and $1,150$ French terms (version of the database of 12/22/2020)\cite{datasetvago2021}. The English lexicon is comprised 95\% of adjectives, all in the classes $V_D$ and $V_C$, the whole vocabulary being distributed as follows: $|V_A|= 8$, $|V_G|= 14$, $|V_D|= 35$ and $|V_C|= 1,470$. Hence 96\% of the English lexicon consists of $V_C$ items. The French lexicon is comprised 97\% of adjectives, again all in the categories $V_D$ and $V_C$. In French, we have $|V_A|= 7$, $|V_G|= 15$, $|V_D|= 28$ and $|V_C|= 1,100$. Accordingly, 96\% of the French lexicon consists of $V_C$  vocabulary. Although the corpora used contained mostly English sentences, they included some French excerpts, which were included for analysis. Hence part of the French lexicon was used.

%While the corpora used contained mostly English sentences, they sometimes included some French excerpts, which were included for analysis.

%\textcolor{blue}{PE: Conflict with Figure 6: this is not the database that was used. In need of correction}

%\textcolor{blue}{BI: But the lexicon used for this experiment also consisted of $1,1150$ French terms now including 97\% of adjectives, again all in the categories $V_D$ and $V_C$. In French, we have $|V_A|= 7$, $|V_G|= 15$, $|V_D|= 28$ and $|V_C|= 1,100$. Accordingly, 96\% of the lexicon consists of $V_C$  vocabulary.}

%The categories $V_A$ and $V_G$ actually contain no adjective but only determiners and modifiers.

%We used the version of the database of 12/22/2020. 

%Version 22-12-2020 de la base de termes 

% EN ANGLAIS :
% TOTAL : 1527 termes

% V_A = 14 termes au total, dont 14 non-adjs (=> 0.52% de non-adjs V_A sur les 1527 termes).

% V_G = 8 termes au total, dont 8 non-adjs (=> 0.92% de non-adjs V_G sur les 1527 termes).

% V_D = 35 termes au total dont 10 non-adjs (=> 28.6% de non-adjs sur les 35 termes V_D, et 0.65% de non-adjs V_D sur les 1527 termes).

% VC = 1470 au total dont 49 non-adjs (=> 3.3% de non-adjs sur les 1470 termes VC, et 3.2% de non-adjs VC sur les 1527 termes)

%Pourcentage de non-adjs sur le total des 1527 termes: 5.3%, donc 94.7% d'adjs. 



% EN FRANCAIS :
% TOTAL : 1150 termes

% V_A = 7 termes au total, dont 7 non-adjs (=> 0.6 % de non-adjs V_A sur les 1150 termes).

% V_G = 15 termes au total, dont 15 non-adjs (=> 1.3 % de non-adjs V_G sur les 1150  termes).

% V_D = 28 termes au total dont 8 non-adjs (=> 28.6% de non-adjs sur les 28 termes V_D, et 0.69% de non-adjs V_D sur les 1150 termes).

% VC = 1100 dont 1100 adjs (95.7 % du total des 1150  termes)

% Total de non-adjs sur les 1150 termes : 30 (2.6%), donc 1120 adjs ( 97.4%)



% \subsection{Validation of the classifier on unseen data}

% The training dataset of the deep learning classifier consists of the four corpora listed above (ISOT-True, ISOT-Fake, SignalMedia1M, Kaggle). Figure \ref{fig:clf_results_per_source} presents the measure of the model performance with respect to the four corpora. The y-axis is the output score; 0 means \textit{``informative"} while 1 stands for a \textit{``biased''} content. The x-axis shows the source corpora. The letter-value plots illustrate the distribution of articles that were part of the test dataset (and thus, excluded from the training).\footnote{The widest box stretches between the first and last quartiles, the second widest boxes stretch between the first/last quartile and the first/last octile, the third widest boxes stretch between the first/last octile and the first/last hexadeciles, etc \cite{letter-value-plot}.}\textcolor{blue}{Not clear how many texts were used as training, how many as test? To be clarified}

% The first two corpora are two facets of the ISOT dataset. Informative or legitimate articles, labeled as ``true news'', and biased articles, labeled as ``fake'', are very well recognized and separated. The same trend is also remarkable in separating SignalMedia1M and Kaggle's datasets, even though \textcolor{blue}{the latter} shows a fuzzier distribution. Overall the classification performance on these {test} datasets results in an F1-score $= 0.955$, indicative of high accuracy. %\textcolor{blue}{PE: Add a word here to say how significant this is; why should "test" be in itaclis as it was before?}% Paul E: what does it mean

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.49\textwidth]{figures/clf_results_per_source.pdf}
%     \caption{Classification of source corpora in the \textit{test} dataset as \textit{informative} (0) or \textit{biased} (1) by \fake.\textcolor{blue}{Figure could be improved: legitimate texts could be grouped left, and biased right? or same color code as below could also be used instead of separate color for each corpus?} %(letter-value plots)
%     }
%     \label{fig:clf_results_per_source}
% \end{figure}

\subsection{Comparison and correlation of \vago and \fake}

%It is intuitive to see a relation between manipulative articles and the presence of vague vocabulary. 

We measure the relation between vagueness and how much articles are predicted to be manipulative by \fake by looking at two classes of vague items detected by \vago, including: all vague items ($V_A + V_G + V_D + V_C$), and subjective vague items ($V_D + V_C$). %\textcolor{red}{and factual vague items ($V_A+V_G$)}.
%With regards to these two classes, Figure \ref{fig:vago_sentences_ratio} displays the score distributions of texts detected by \fake as \textit{legitimate} (in blue) and \textit{biased} (in red).

The relation between articles predicted to be manipulative and the presence of vagueness is measured in Figure \ref{fig:vago_sentences_ratio}~a), using \vago as our detector of vague sentences, and the measure reported in Eq. (\ref{eq:prop_vague}) for vagueness. On the left hand side, the x-axis shows the predicted class (\textit{legitimate} in blue, \textit{biased} in red) by \fake. The y-axis displays the percentage of sentences containing markers of vagueness (the higher, the more vague). The Pearson correlation coefficient between these two variables (\textit{biased}, and \textit{vague}) is 0.208 (sample size $=28,692$): \textit{biased} articles tend to contain more vague sentences, but vagueness is not the sole determining factor.

%% Comment 1 by Paul: should we also report the p-value for the correlation test? At least indicate number of data points for effect size

%% Comment 2 by Paul: do I understand correctly that in each text you calculate sentence by sentence whether R_vague(phi)>0, and then you just look at the proportion of vague sentences in text? Note that this is different from the measure we suggest in (3) above, but corresponds to (5). Maybe we can do both, in that case we should also give the measure you propose for the degree of vagueness in a text. Same comment for subjectivity below ie (6) vs (4)

%% Answer 2 by Paul G: that's correct. I have displayed figures corresponding to formula (5). Figures corresponding to formula (3) are not displayed to avoid clutter, but are available in the figures directory.

%A split according to the type of vagueness provides some insights on Figure \ref{fig:vago_sentences_ratio}~b). 


%Both ISOT corpora reveal similar vague ratios; signalmedia is generally more precise; kaggle tends to have more vague sentences. Moreover it contains some very precise articles with very low vague scores (inferior to 0.20).

%% Comment Paul: how can we explain that ISOT true and false have the same vagueness ratio? That they have more vagueness than kaggle?

%% Answer Paul G: As suggested during the April 9th call, both isot have similar vague score, however isot_fake is has more vague-subj whereas isot_true has more vague-factual. It is shown in what is now Fig 5.

A similar analysis is performed using VAGO as a detector of \textit{subjective} sentences, also described as opinion sentences, using the measure of subjectivity reported in Eq. (\ref{eq:prop_subj}); this analysis is displayed in Figure \ref{fig:vago_sentences_ratio}~b). There, the y-axis displays the ratio of sentences that contain $V_C$ and $V_D$ type keywords. Here the correlation between these two variables is 0.271: articles detected as \textit{biased} tend to contain more markers of subjectivity.

% \textcolor{red}{
% To lay stress on the role of $V_G$ and $V_A$ keywords, a third analysis is performed using VAGO as a detector of \textit{factual vagueness}, \textit{i.e.} sentences containing markers of factual-vagueness but no markers of subjective vagueness. The score of factual-vagueness of a sentence is calculated as follows.}
% \textcolor{red}{
% \begin{equation}
% R_{factual-vague}(\phi) =
%     \begin{cases}
%     0 & \text{if } R_{subjective}(\phi) > 0 \\
%     \frac{|V_G|_{\phi} + |V_A|_{\phi}}{N_{\phi}} & \text{otherwise}
%     \end{cases}
% \end{equation}
% }

% \textcolor{red}{\noindent Similarly to Eq. (\ref{eq:prop_subj}), the global factual-vagueness score of a text is given by:}

% \textcolor{red}{
% \begin{equation}\label{eq:fv}
% R'_{factual-vague}(T)=\frac{|\{\phi \in T | R_{factual-vague}(\phi)>0\}|}{N_T}
% \end{equation}
% }

% \textcolor{red}{\noindent This analysis is displayed in Figure \ref{fig:vago_sentences_ratio}~c). The Pearson correlation between the two variable is -0.075. Texts detected as informative have a slight tendency to contain more vague sentences with no markers of subjectivity.}

\begin{figure}[htbp]
    \footnotesize
    \begin{tabular}{cc}
        a. & \!\!\!\!\!\!\!\! \includegraphics[align=c,width=0.94\columnwidth]{figures/vago_vague_sentences_ratio_cropped.png} \\
        b. & \!\!\!\!\!\!\!\! \includegraphics[align=c,width=0.94\columnwidth]{figures/vago_opinion_sentences_ratio.png}
    \end{tabular}
    
    \caption{Comparison between \fake predictions and (a) ratio of vague sentences, (b) ratio of subjective sentences
    %and ratio of vague-factual sentences (c) 
    in texts, as predicted by \vago.}
    \label{fig:vago_sentences_ratio}
\end{figure}

% what about fig:vago_sentences_ratio C) ??


A split according to the source corpora provides further insights. Regarding subjectivity, Figure \ref{fig:distrib_vague_sources}~b) shows that corpora follow the tendency of their \textit{legitimate} vs. \textit{biased} affiliation: ISOT-true and SignalMedia1M texts are detected as less subjective than ISOT-fake and Kaggle texts. While ISOT-true documents and ISOT-fake documents contain the same proportion of vague terms all types included (Figure \ref{fig:distrib_vague_sources}~a), the difference between them concerns the occurrence of subjective vocabulary (Figure \ref{fig:distrib_vague_sources}~b). 

%However, Figure \ref{fig:distrib_vague_sources}~a) exhibits a break in this tendency: ISOT-true documents are detected as sensibly as vague as ISOT-fake documents. 

%A post hoc analysis indicates that the ISOT-True corpus contains a higher-rate of vague sentences of type $V_A$ and $V_G$ than the ISOT-False

%Figure \ref{fig:distrib_vague_sources}~c) reveals that this is due to the high rate of \textit{factual-vague} sentences in ISOT-true.



\begin{figure}[htbp]
    \scriptsize
    \begin{tabular}{cm{.05\columnwidth}cm{.9\columnwidth}}
        a. & \includegraphics[width=0.9\columnwidth]{figures/vago_vague_sentences_ratio_sources.pdf} \\
        b. & \includegraphics[width=0.9\columnwidth]{figures/vago_opinion_sentences_ratio_sources.pdf} \\
        % c. & \includegraphics[width=0.9\columnwidth]{figures/vago_vaguefactual_sentences_ratio_sources.pdf} \\
    \end{tabular}
    
    \caption{Distribution of vague sentences ratio (a), vague-subjective sentences ratio (b) %and vague-factual sentences ratio (c) 
    across sources.}
    \label{fig:distrib_vague_sources}
\end{figure}

% To summarize, the prevalence of subjective vocabulary can be seen as a predictor of fake texts.
% However, vagueness is not necessarily paired with illegitimacy, as seen in ISOT-true.
% Overall, ISOT-fake is the source with the most subjective texts. However, even if the correlation between bias and subjectivity is larger (0.271), the sole subjectivity ratio is not sufficient to detect biased articles.

\subsection{Word-level analysis: exploiting the deep to find new keywords}

\fake not only provides a prediction at article-level, but also a word-level contextual score to enable an understanding of its predictions. In Figure \ref{fig:category_distrib} we display the distribution of the average ``fakeness'' score (the CAM word-level score) of the occurring \vago keywords, as they are perceived by the classifier.
%We propose to display in Figure \ref{fig:category_average} the average bias or fakeness score of the VAGO keywords, as they are perceived by the classifier. 
Each dot represents the average ``fakeness'' score of a vocabulary entry across all its occurrences. For each category, a boxplot sums up the score distribution.
$V_A$ and $V_G$ words used to identify \textit{vague-factual} sentences are in blue; $V_C$ and $V_D$ words used to identify \textit{vague-subjective} sentences are in red. Gray bars give the scores for other adjectives and adverbs, as a reference, as \vago contains mostly adjectives. Non-\vago entries have been tagged as adjectives or adverbs by jointly using TextBlob\footnote{\url{https://github.com/sloria/TextBlob}} and NLTK part-of-speech tagging.
% The $V_A$ category contains only nine entries encountered in the test dataset. The $V_C$ category is the most abundant in the \vago vocabulary. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/category_distrib.pdf}
    \caption{Average ``fakeness'' scores of \vago entries and other adjectives and adverbs according to \fake class attention maps, defined in Equation~\ref{eq:CAM-definition}.}
    \label{fig:category_distrib}
\end{figure}

% Figure~\ref{fig:category_distrib} gathers the average CAM scores of \vago and some non-\vago vocabulary entries.

As described in section \ref{sec:cam}, for every token in a sentence the CAM provides a signed score accounting for the contribution of this token and its near context to the prediction of the whole sentence. Thus, we consider that a high CAM score stands for a highly bias-inducing word according to \fake. We can see from this figure that belonging to a vague category is not sufficient to trigger a \textit{biased} or \textit{legitimate} label; however some words remain good cues in that respect. In Table \ref{tab:fakest_adjectives}, we propose a list of the thirty most bias-inducing adjectives and adverbs (considering the prevalence of adjectives in \vago and the proximity of adverbs to adjectives). The first two columns present the number of occurrences of each term and its average ``fakeness'' score. The third gives the semantic type (when listed in \vago) and the fourth the syntactic category.

\begin{table}[htbp]
    \centering
    \begin{tabular}{c|ccccc}
            word & occ & avg & \vago & part-of-speech \\ \hline
            
        \textbf{sociable} & 32 & 80.42 & V\textsubscript{C} & adj.\\
        \textbf{disgusting} & 231 & 61.50 & V\textsubscript{C} & adj.\\
        \color{gray!50}stumble & \color{gray!50}28 & \color{gray!50}57.28 & \color{gray!50} & \color{gray!50}adj.\\
        Orwellian & 13 & 44.69 &  & adj.\\
        sociopathic & 12 & 42.40 &  & adj.\\
        arrogantly & 13 & 42.04 &  & adv.\\
        misogynistic & 37 & 41.84 &  & adj.\\
        entire & 2246 & 41.54 &  & adj.\\
        \textbf{idiotic} & 48 & 40.86 & V\textsubscript{C} & adj.\\
        courageously & 15 & 40.43 &  & adv.\\
        neoconservative & 25 & 40.30 &  & adj.\\
        % \textbf{pailful} & 1 & 39.62 & V\textsubscript{C} & noun\\
        neoliberal & 45 & 39.31 &  & adj.\\
        coincidentally & 24 & 37.52 &  & adv.\\
        subliminal & 14 & 36.81 &  & adj.\\
        % \textbf{insinuating} & 3 & 36.51 & V\textsubscript{C} & adj.\\
        \textbf{delusional} & 61 & 35.78 & V\textsubscript{C} & adj.\\
        \textbf{pitiful} & 18 & 35.43 & V\textsubscript{C} & adj.\\
        % \textbf{foolproof} & 6 & 35.09 & V\textsubscript{C} & adj.\\
        frighteningly & 10 & 34.78 &  & adv.\\
        disturbingly & 16 & 34.30 &  & adv.\\
        shamelessly & 26 & 34.08 &  & adv.\\
        blatantly & 75 & 33.92 &  & adv.\\
        \textbf{astonishing} & 100 & 33.62 & V\textsubscript{C} & adj.\\
        laughably & 11 & 33.56 &  & adv.\\
        \color{gray!50}sic & \color{gray!50}101 & \color{gray!50}33.21 & \color{gray!50} & \color{gray!50}adj.\\
        outrageously & 18 & 32.67 &  & adv.\\
        \textbf{racist} & 971 & 32.27 & V\textsubscript{C} & adj.\\
        % \textbf{responsable} & 9 & 32.26 & V\textsubscript{C} & adj.\\
        \textbf{massive} & 1314 & 32.14 & V\textsubscript{C} & adj.\\
        devious & 13 & 31.81 &  & adj.\\
        transnational & 52 & 31.73 &  & adj.\\
        \textbf{deplorable} & 85 & 31.56 & V\textsubscript{C} & adj.\\
        Siberian & 11 & 31.51 &  & adj.\\
        % \textbf{moronic} & 15 & 31.30 & V\textsubscript{C} & adj.\\
        % \textbf{une} & 17 & 30.65 & V\textsubscript{G} & article (Fr)\\
        % treasonous & 26 & 30.29 &  & adj.\\
        % sexually & 300 & 30.26 &  & adv.\\
        % unhinged & 63 & 30.11 &  & adj.\\
        % \textbf{aimable} & 2 & 30.09 & V\textsubscript{C} & adj. (Fr)\\
        
    \end{tabular}
    \caption{Thirty most bias-inducing terms according to \fake, filtered to adjectives and adverbs with at least 10 occurrences. Entries are sorted by descending average CAM scores (avg column). \vago terms are in bold. Miscategorized adjectives and adverbs are in gray. %\textcolor{blue}{PE: expressions in "should" are not adverbial or adjectival, to be clarified}
    }
    \label{tab:fakest_adjectives}
\end{table}
  
  
  
\begin{table}[htbp]
    \centering
    \begin{tabular}{c|ccccc}
            word & occ & avg & \vago & part-of-speech \\ \hline

        \color{gray!50}Carly & \color{gray!50}16 & \color{gray!50}-60.89 & \color{gray!50} & \color{gray!50}adj.\\
        \color{gray!50}Emily & \color{gray!50}72 & \color{gray!50}-60.84 & \color{gray!50} & \color{gray!50}adv.\\
        provisionally & 28 & -58.53 &  & adv.\\
        40th & 32 & -53.64 &  & adj.\\
        \color{gray!50}Experian & \color{gray!50}40 & \color{gray!50}-48.58 & \color{gray!50} & \color{gray!50}adj.\\
        \color{gray!50}vSphere & \color{gray!50}14 & \color{gray!50}-47.59 & \color{gray!50} & \color{gray!50}adv.\\
        upwardly & 11 & -46.20 &  & adv.\\
        fortnightly & 11 & -46.13 &  & adv.\\
        \textbf{cloudy} & 99 & -44.04 & V\textsubscript{C} & adj.\\
        sectoral & 14 & -43.56 &  & adj.\\
        unbeaten & 113 & -42.26 &  & adj.\\
        \color{gray!50}trimble & \color{gray!50}19 & \color{gray!50}-41.68 & \color{gray!50} & \color{gray!50}adj.\\
        \color{gray!50}premiere & \color{gray!50}57 & \color{gray!50}-40.97 & \color{gray!50} & \color{gray!50}adv.\\
        \color{gray!50}Sebastian & \color{gray!50}80 & \color{gray!50}-38.96 & \color{gray!50} & \color{gray!50}adj.\\
        directorial & 12 & -37.21 &  & adj.\\
        playable & 18 & -37.18 &  & adj.\\
        Tanzanian & 11 & -36.07 &  & adj.\\
        treble & 19 & -36.01 &  & adj.\\
        undertaken & 25 & -35.82 &  & adj.\\
        interactive & 378 & -35.57 &  & adj.\\
        \color{gray!50}semifinal & \color{gray!50}19 & \color{gray!50}-34.96 & \color{gray!50}  & \color{gray!50}adj.\\
        topographic & 16 & -34.77 &  & adj.\\
        shareable & 10 & -34.44 &  & adj.\\
        \color{gray!50}Dorian & \color{gray!50}10 & \color{gray!50}-33.97 & \color{gray!50} & \color{gray!50}adj.\\
        procedural & 92 & -33.50 &  & adj.\\
        \textbf{muddy} & 46 & -33.48 & V\textsubscript{C} & adj.\\
        unrivalled & 13 & -33.24 &  & adj.\\
        \textbf{comprehensive} & 1001 & -32.52 & V\textsubscript{C} & adj.\\
        \textbf{moody} & 146 & -32.37 & V\textsubscript{C} & adj.\\
        unauthorised & 14 & -32.36 &  & adj.\\
        % presbyterian & 21 & -32.27 &  & adj.\\
        % organisational & 23 & -32.24 &  & adj.\\
        % \textbf{juste} & 1 & -32.22 & V\textsubscript{C} & adj. (Fr)\\
        % victorian & 120 & -32.16 &  & adj.\\
        % \textbf{languid} & 8 & -32.03 & V\textsubscript{C} & adj.\\
        % \textbf{geeky} & 12 & -32.00 & V\textsubscript{C} & adj.\\
        % incisive & 11 & -31.91 &  & adj.\\
        % \color{gray!50}archdiocese & \color{gray!50}10 & \color{gray!50}-31.89 & \color{gray!50} & \color{gray!50}adj.\\
        % \textbf{scornful} & 5 & -31.64 & V\textsubscript{C} & adj.\\
        % gorgeously & 10 & -31.64 &  & adv.\\
    \end{tabular}
    \caption{Thirty least bias-inducing terms  according to \fake, filtered to adjectives and adverbs with at least 10 occurrences. Entries are sorted by ascending average CAM scores (avg column). \vago terms are in bold. Miscategorized adjectives and adverbs are in gray.%\textcolor{blue}{Several corrections to make here.}%\textcolor{blue}{not sure that we should keep this table, "should'' does not appear in the database version we describe in section IV, and is not an adjectival or adverbial phrase; we need to clarify which version of database was used}
    }
    \label{tab:legitest_adjectives}
\end{table}
  
  
  Even though two part-of-speech tagging tools were used to identify ``other  adjectives''  and  ``other adverbs'', some artifacts (displayed in gray) are wrongly tagged as adjectives or adverbs. Several evaluative adjectives like
 ``disgusting'' and ``racist'' are identified by \vago as markers of subjectivity; others like ``Orwellian'', ``sociopathic'' and ``arrogantly'' are not in the \vago database but are also clear vehicles of subjectivity and evaluativity. In fact, disregarding the two artifacts marked in gray, all terms in Table \ref{tab:fakest_adjectives} are adjectives or adverbs that fall under the category of combinatorial vagueness and that could be added as such to the \vago lexicon.
 
 %These terms indeed fall into the category of combinatorial vagueness and are good candidates to be added into the \vago vocabulary.
 
A comparison with least bias-inducing terms (scores ranging $[-60; -30]$, Table \ref{tab:legitest_adjectives}) shows a more heterogeneous set. Fewer terms are already part of the \vago lexicon. Furthermore, among adjectives and adverbs, several are non-gradable and precise (``40th'', ``unbeaten'', ``upwardly'', ``fortnightly'', ``Tanzanian'', ``unauthorized''). Fewer correspond to evaluative adjectives or to adjectives that would be eligible for the type $V_C$ (``interactive'', ``unrivalled'' may be exceptions).

%(``procedural'' might be an exception).
  
% This analysis is not reproducible in the same way for the most legitimate terms (Table \ref{tab:legitest_adjectives}): ``invitational'', ``provisionally'', ``fortnightly'' or ``interactive'' (scores ranging $[-80; -40]$) do not bear as much information as their biased counterparts. This suggests that while vague-subjective words can signal bias in text, factual discourse is not attached to specific lexical markers.

%This suggests that, while one word is enough to add bias in a factual sentence, the opposite does not stand. % "classe naturelle" ?

% @Guillaume: j'ai ajouté 2 CSV dans /data (fakest200.csv et legitest200.csv). Ils contiennent les 200 mots [VAGO + autres adjectifs >= 10 occurrences  + autres adverbes >= 10 occurrences] triés par score moyen descendant (fakest) et ascendant (legitest).

==> FUSION_ expert-based Vago and deep-based FakeClf for desinfo/texts/5discussion.tex <==
%% section discussion



%% Paul: start with summary of hypothesis and results

Our hypothesis in this paper was that because vague terms are often subjective, the prevalence of vagueness in discourse can be used as a cue that the discourse conveys fake news (whether \emph{biased} or \emph{bullshit}). In order to test this hypothesis, we pooled two distinct methodologies. The first methodology involved the semantic-based algorithm \texttt{VAGO}, which provides a measure of vagueness vs precision in text, and a measure of subjectivity vs objectivity in text. The second methodology involved the deep-learning classifier \fake, relying on CNN and CAM techniques. 

By comparing the results of \fake with the measures of vagueness and subjectivity obtained by \vago on four distinct corpora pre-identified as containing ``fake'' vs ``true'' articles, we found a positive correlation between vagueness and fakeness, as well as between subjectivity and fakeness. The association with fakeness is stronger for subjective vague terms (of type $V_D$ and $V_C$ in \vago's taxonomy). While an overwhelming majority of the terms in the \vago database are markers of subjectivity, this stronger association also confirms that not all types of vagueness introduce subjectivity.
% By comparing the results of \fake  with the measures obtained by \texttt{VAGO} on four distinct corpora tagged manually as ``fake'' or ``legitimate'', we found that a) biased corpora contain more vague sentences than legitimate corpora, b) biased corpora contain more subjective vague sentences than legitimate corpora, which tend to be more factual. In particular, a) the biased corpora Isot-fake and Kaggle contain more vague sentences than the legitimate corpora Isot-true and SignalMedia1M. And b) the biased corpora Isot-fake and Kaggle contain more subjective vague sentences than the legitimate corpora Isot-true and SignalMedia1M.

% While the correlation found between the vagueness and subjectivity measures and the classification of texts as biased or legitimate is small (around 0.25), it lends support to our main hypothesis. Furthermore, the \texttt{VAGO} taxonomy predicts that not all vague terms are subjective. What was found is that subjective vagueness is indeed a better predictor of fakeness than vagueness taken indistinctly. 

From a methodological point of view, the two approaches discussed in this paper can be viewed as complementary. In one direction, \fake identifies as markers of fakeness some adjectives not originally in the \texttt{VAGO} database, but which clearly belong to the class $V_C$ of adjectives exemplifying multi-dimensional vagueness, and conveying subjectivity. The correlation found is therefore expected to increase by the inclusion of a larger vocabulary.
In the converse direction, the typology deployed in \texttt{VAGO} helps to make the results of \fake more easily interpretable and explainable. Indeed, while the inductive generalizations operated by \fake remain opaque, \texttt{VAGO} rests on a transparent semantic architecture. More work is needed to narrow the gap between the two approaches, but the consistency in the correlation between the two classifications is a step toward increased explainability.

% Finally, we saw that extensions of the \texttt{VAGO} database to grammatical categories other than adjectives and adverbs also receives some light from \fake. Beside adjectives, the authors of \texttt{VAGO} had made the specific conjecture that the modal auxiliary ``should'' may also introduce vagueness and subjectivity in discourse, based on the occurrence of ``should'' in a variety of non-factual moral claims. Interestingly, the results of \fake suggest that ``should'' is also found in ``legitimate'' texts, and is not a reliable marker of vagueness. This makes sense, since ``should'' also supports epistemic interpretations, compatible with factual reports. The use of Fake-Clf thus allows us to control and refine the semantic typology gradually deployed in \texttt{VAGO}. 


%% PE= A réécrire

%Finally, we noted that the words most frequently found in ``legitimate'' corpora do not appear to form a natural class, neither from a grammatical nor from a semantic point of view. While this result should be taken with care, it lends support to the idea that objectivity is more adequately characterized as the absence or minimization of subjective terms than by the occurrence of a specific vocabulary.

%, (this is more clear for isot-fake. 


%%%%

% Hypothesis

% Fig 4:  Fake-Clf applied to Vago pre-classification

% a) biased corpora contain more vague sentences than legitimate corpora, b) biased corpora contain more subjective vague sentences than legitimate corpora, that tend to be more factual

%This confirm the Vago classification

%Results are replicated on the four sources of corpora. 

%Figure 5 :  Fake-Clf applied to the four sources of corpora 

% a) Biased corpora isot-fake and Kaggle contain more vague sentences than legitimate corpora isot-true and SignalMeddia; b)  Biased corpora isot-fake and Kaggle contain more subjective vague sentences than legitimate corpora isot-true and SignalMeddia (this is more clear for isot-fake). 



%% Discuss the promising aspects

%% Discuss the sense in which the results can be fed back into VAGO and why they confirm the classification

%% Discuss also the false negatives

%% Discuss the issue of explainable IA in relation to this


%% Ghislain: take also into account that some rules in VAGO (such as [num] + [tall/long ] that remove degree vagueness. Such rules are implemented but how to recognize those patterns in DL?

%% what about the rule [SHOULD + VERB => combinatory vagueness? 
%A recent survey on explainable AI \cite{adadi2018peeking} divided its benefits into four topics: justify, control, improve, and discover. Following this suggestion, we propose the following list of opportunities.
%% see data all_vago_output_expe_terms.csv
%% output eval of terms 655 : should + [VERB]
% 1796: total VC total: 1 141 termes VC wihtout the rule SHOULD + [VERB] 

%POINTS DE CONCLUSION PE (added by BI):

%1) Contrairement à la subjectivité, on observe qu'il n'y a pas d'homogénéité dans les marqueurs de la factualité (ie tout ce qui n'est pas subjectif est factuel derechef). Dit autrement : pas de symétrie entre les catégories "factuel" et "subjectif" dans notre typologie

%2) a) dire que les résultats actuels assoient la taxonomie et montrent l'intérêt d'avoir une taxonomie : toutes les fake news ne sont pas trompeuses de la même manière, il y a différentes catégories de fake news 

%Mais b), révision, add-on sur la taxonomie : peut-être a-t-on marqué trop rapidement certains termes dans la taxonomie vago existante (ex: "should") 

%3) Fusion perspective: how to combine both methodological approaches (Vago + FakeClf) to obtain more adequate results. 

%Complementarity of these approaches: to improve one another, and to bring perspective. Explain how the CLF identifies vague adjectives not initially in the database. So how we might improve the correlation simply by enlarging the database (suggesting the experts to choose more keywords).

%4) Other paths to improve the detection : deduce the \textbf{attitude} and intention of the speaker, through its use of manipulative phrases and vague semantics. 

%5) Put some lights on explanability of AI

% Explainability: remind that VAGO is completely transparent; whereas Fake-CLF is "half-transparent", thanks to the cams.

% Necessity to have an explanation in the fake news domain (as fakes exist also because the ``official media'' are not accepted, not trusted).








==> FUSION_ expert-based Vago and deep-based FakeClf for desinfo/texts/6conclusion.tex <==
%%% summary of the proposal and results obtained
%% limitations 
%% future work

Focusing on lexical vagueness as a marker of subjectivity, we have combined a semantic-based NLP engine \vago with a deep-learning classifier \fake to improve the detection of fake news contents. %Both approaches not only agree on classification results but 
The two approaches yield convergent results and they each provide useful input to improve the other. 

Several points remain for further elaboration. First of all, the \vago lexicon was still limited at the time of this comparison. We have seen how it can be expanded using \fake, but the base will keep evolving. %In particular, here the vague lexicon consists mostly of adjectives, and the present study confirms that adjectives are typical bearers of subjectivity and evaluativity \cite{Kaiser&Wang2021}.
In particular, other expressions beside adjectives (and adverbs) can introduce vagueness and subjectivity. One non-adjective that was included in \vago at the time of this comparison is the modal ``should''. ``Should'' was tentatively classified as $V_C$ considering its expressive dimension in  deontic utterances stating moral prescriptions. As it turns out, \fake predicts that ``should'' is not among the most bias-inducing terms when more entries than adjectives and adverbs are considered for analysis. Further work is needed to adjudicate the potential vagueness and subjectivity of ``should'' and related modals.

%, consistently with ``should'' having epistemic readings. %% Words in should are highly represented in the least-bias inducing

Secondly, the correlation found between \textit{biased} predictions and subjectivity scores is limited, thus subjectivity explains only part of the variance in the classification of \fake. This is not surprising, since subjectivity is only one among several factors that can contribute to misinformation. Fake news consist not only in opinionated texts, but also in clever fabrications, hoaxes, or simply mistaken factual reports \cite{rubin2015deception}. The type of integration proposed between \fake and \vago should therefore be extended to explore other sources of fakeness beside bias.

%POINTS CONCLUSION :

%How can Fake-Clf help improve Vago ?


% Conversely, how can Vago help improve Fake-Clf ?


%POINTS CONCLUSION :

% 1) Elargir la base VAGO 

% 2) Mention other sources of fakeness: not just vagueness, but more dimensions.

% Other markers: not just adjectives and adverbs. More categories to be addressed.

% Mention enlargement of VAGO database

% Mention how VAGO could help the classifier to improve thanks to external vocabulary
%

%



